Giant non-equilibrium fluctuations in diffusion in freely-suspended liquid films

Experimental work has shown that non-equilibrium concentration fluctuations arise during free diffusion in fluids and theoretical analysis has been carried on. The results show that, in usual three-dimensional fluids, the phenomenon is extremely weak, in terms of amplitude of the fluctuations and of corrugation of the diffusion wave fronts. In this paper, we show that the phenomena strongly depends on the dimensionality of the system: by extending the theory to two dimensional systems, we show that the root mean square amplitude of the fluctuations and the wave front corrugation become much stronger. We also present an evaluation of the Hausdorf dimension of the expected fluctuations. Experimentally, two-dimensional liquid systems can be realised as freely suspended liquid films; experiments and theoretical works on diffusion in such systems showed that the dynamics is deeply affected by the viscous drag exerted by the fluids (e.g. air) surrounding the film. We provide an evaluation of the drag on the fluctuations. In particular, we study the case of a concentration profile that is initially gaussian: it can be directly compared with the results from a fluorescence recovery after photobleaching (FRAP) experiment. We propose that this theory and the related experiments can be relevant for describing the diffusion along the cellular membranes of living organisms.

==> Makefile <==
TESTO=2d

all : $(TESTO).pdf
	evince $(TESTO).pdf
	pdftotext $(TESTO).pdf
	cat $(TESTO).txt | sed 's/[0-9]*//g' | wc -w

dependencies.d : $(TESTO).tex
	printf "$(TESTO).pdf: $(TESTO).bib " >dependencies.d
	perl -e 'for (<STDIN>) { if (/% require (.+)/) { print " $$1"; } }' <$(TESTO).tex >>dependencies.d

-include dependencies.d

%.pdf : %.tex dependencies.d
	-gnuplot $$(basename $< .tex)1.gp
	for nome in $$(find . -empty -name "$$(basename $< .tex)1_*.eps"); do rm $$nome; done
	-cp $$(basename $< .tex)1.gp fatto.gp
	touch fatto.gp
	pdflatex -interaction=batchmode $<
	-gnuplot $$(basename $< .tex)1.gp
	for nome in $$(find . -empty -name "$$(basename $< .tex)1_*.eps"); do rm $$nome; done
	-if ! diff $$(basename $< .tex)1.gp fatto.gp -q; then pdflatex -interaction=batchmode $<; fi
	-bibtex $$(basename $< .tex)


%.eps : %.fig
	fig2dev -L eps $< $@

%.eps : %.jpg
	jpegtopnm $< >memo.pnm
	pnmscale -pixels 140000 memo.pnm >memo1.pnm
	pnmtops -imagewidth 3 -noturn memo1.pnm >$@
	rm memo.pnm memo1.pnm

%.eps : %.odg
	libreoffice --headless --convert-to pdf $<
	pdftops $$(basename $< .odg).pdf
	mv $$(basename $< .odg).ps $@
	rm $$(basename $< .odg).pdf

%.eps : %.ods
	libreoffice --headless --convert-to pdf $<
	pdftops $$(basename $< .ods).pdf
	mv $$(basename $< .ods).ps $@
	rm $$(basename $< .ods).pdf

prussian_blue :
	povray -H1000 -W1000 prussian_blue.pov
	povray -H1000 -W1000 prussian_blue_key.pov

%.txt : %.cpp
	g++ -o esegui_memo $< -lm -lgsl -lgslcblas
	./esegui_memo >$@
	rm esegui_memo

doc: $(TESTO).pdf prepara_spedizione
	cp $(TESTO).pdf README.txt /home/dbrogioli/Dropbox/libro\ SGP/
	cp spedizione/spedizione.zip  /home/dbrogioli/Dropbox/libro\ SGP/sources.zip

odt :
	-rm -rf odtdir
	mkdir odtdir
	perl rtf.pl libro >odtdir/libro.tex
	-cp libro.bbl odtdir
	-cp *.sty odtdir
	export TEX4HTENV=/etc/tex4ht/tex4ht.env; cd odtdir; latex libro.tex; latex libro.tex; mk4ht oolatex libro.tex; cp libro.odt /home/dbrogioli/Dropbox/libro\ SGP/; libreoffice libro.odt



prepara_spedizione :
	-rm -rf spedizione
	mkdir spedizione
	mkdir spedizione/testo
	perl spedizione.pl $(TESTO)
	cd spedizione/testo; zip ../spedizione.zip *
	cp -r spedizione/testo spedizione/prova
	#cp *.bst spedizione/prova
	#cp *.clo spedizione/prova
	#cp *.cls spedizione/prova
	cd spedizione/prova; latex $(TESTO).tex; pdflatex $(TESTO).tex; bibtex $(TESTO); pdflatex $(TESTO).tex; pdflatex $(TESTO).tex; evince $(TESTO).pdf



clean :
	-rm $(TESTO).dvi $(TESTO).ps $(TESTO).aux $(TESTO).log $(TESTO).pdf $(TESTO).bbl $(TESTO).blg $(TESTO).d 
	-rm *.eps
	-rm *~
	-rm *.bak
	-rm $(TESTO)1.gp

